Secretary Ranking with Minimal Inversions

We study a twist on the classic secretary problem, which we term the secretary ranking problem: elements from an ordered set arrive in random order and instead of picking the maximum element, the algorithm is asked to assign a rank, or position, to each of the elements. The rank assigned is irrevocable and is given knowing only the pairwise comparisons with elements previously arrived. The goal is to minimize the distance of the rank produced to the true rank of the elements measured by the Kendall-Tau distance, which corresponds to the number of pairs that are inverted with respect to the true order. Our main result is a matching upper and lower bound for the secretary ranking problem. We present an algorithm that ranks $n$ elements with only $O(n^{3/2})$ inversions in expectation, and show that any algorithm necessarily suffers $\Omega(n^{3/2})$ inversions when there are $n$ available positions. In terms of techniques, the analysis of our algorithm draws connections to linear probing in the hashing literature, while our lower bound result relies on a general anti-concentration bound for a generic balls and bins sampling process. We also consider the case where the number of positions $m$ can be larger than the number of secretaries $n$ and provide an improved bound by showing a connection of this problem with random binary trees.

==> abstract.tex <==
\begin{abstract}

We introduce the \emph{online ranking} problem as a generalization of the classical secretary problem. 
Elements $a_1,\ldots,a_n$ are arriving one by one in an online fashion.  Upon arrival of every element $a_i$, we need to irrevocably place $a_i$ in its correct position in the sorted order of all elements, i.e., in the position corresponding to \emph{rank} of $a_i$. More precisely, when $a_i$ arrives, it has to be assigned to a position $\pi(a_i)$ \emph{not yet occupied} in $[n]$. The goal is to minimize the number of \emph{inversions} defined as number of pairs of elements $a_i$ and $a_j$ such
that $a_i < a_j$ but $\pi(a_i) > \pi(a_j)$. Similar to the secretary problem, we make the enabling assumption that the elements are arriving in a \emph{random order}. 

We obtain the first non-trivial upper and lower bounds for this problem. We develop an algorithm for this problem that with high probability outputs
a solution with only $O(n^{5/3})$ inversions. This makes a significant improvement over the trivial upper bound of $O(n^2)$ on the number of inversions. 
We complement our upper bound result by showing that any algorithm for this problem outputs a solution with at least $\Omega(n^{3/2})$ inversions in expectation. 
\end{abstract}


==> problem.tex <==
% !TeX root = ranking.tex

%\renewcommand{\rank}{\ensuremath{\textnormal{\textsc{rank}}}\xspace}

\section{Preliminaries}
\label{sec:prelim}




%\paragraph{Trivial bounds.} As a starting point, we show trivial upper and lower bounds for this objective. First, the cost of any algorithm is at most $\binom{n}{2}$, which is the number of pairs of elements. The random algorithm, which at time $i$ picks rank $\pi(a_{(i)})$ for element $a_{(i)}$ uniformly at random among all the ranks not yet occupied, has expected cost that only improves the worst case cost by a factor of $2$: each pair of element has probability $1/2$ to have the same ordering according to the true and ``learned'' rank. Thus, a trivial upper bound is $O(n^2)$.

%For a lower bound, observe that the probability that the first element to arrive
%is $a_{\sigma(1)}$ with $\sigma(1) \leq n/4$ is $1/4$, which is also the
%probability that $\sigma(1) \geq 3n/4$. These two cases are indistinguishable to
%the algorithm since it does not observe any information about the first element
%to arrive. Thus, the decision $\pi(a_{(1)})$ of the algorithm for rank of the
%first element when $\sigma(1) \in [1, n/4] \cup [3n/4 ,n]$ is independent of
%whether $\sigma(1) \leq n/4$ or $\sigma(1) \geq 3n/4$. Thus, with probability
%$1/4$, the algorithm has cost at least $3n/4 - n/4 = n/2$ and we obtain an
%$\Omega(n)$ lower bound for any algorithm.

